Optimal Power Flow with Step-Voltage Regulators in Multi-Phase Distribution Networks

This paper develops a branch-flow based optimal power flow (OPF) problem for multi-phase distribution networks that allows for tap selection of wye, closed-delta, and open-delta step-voltage regulators (SVRs). SVRs are assumed ideal and their taps are represented by continuous decision variables. To tackle the non-linearity, the branch-flow semidefinite programming framework of traditional OPF is expanded to accommodate SVR edges. Three types of non-convexity are addressed: (a) rank-1 constraints on non-SVR edges, (b) nonlinear equality constraints on SVR power flows and taps, and (c) trilinear equalities on SVR voltages and taps. Leveraging a practical phase-separation assumption on the SVR secondary voltage, novel McCormick relaxations are provided for (c) and certain rank-1 constraints of (a), while dropping the rest. A linear relaxation based on conservation of power is used in place of (b). Numerical simulations on standard distribution test feeders corroborate the merits of the proposed convex formulation.

==> SVRLineDiagram.tex <==
\begin{tikzpicture}
\tikzstyle{LineOut}   = [ draw=black,  thick, o-]
\tikzstyle{LineIn}   = [ draw=black,  thick, -o]
\tikzstyle{LittleArrow}= [draw=black, thin, ->]
\tikzstyle{Block}=[rectangle, draw=black, thick, text width=5em, text centered, sharp corners]
	\node [matrix, ampersand replacement=\&, column sep=12mm, row sep=1mm] (SeriesModels){ 
		\node  (Noden) {$v_n$}; \& \node [Block] (Anm) {$A_{nm}$}; \& \node (Nodem){$v_m$}; \\
		\& \node (Ground) [ground]{}; \& \\
};
\begin{scope}
\path [LineOut](Noden.east) -- node [name=MidwayNodeN, midway, yshift=4mm] {$i_{nm}$}  (Anm.west); 
\path [LineIn](Anm.east) -- node [name=MidwayNodeM, midway, yshift=4mm, color=red] {$i'_{nm}$}  (Nodem.west); 
\draw ($(MidwayNodeN.south)$) node [yshift=-0.5mm] {$\rightarrow$}; 
\draw ($(MidwayNodeM.south)$) node [color=red,yshift=-0.5mm] {$\rightarrow$}; 
\draw  (Anm.south) -- (Ground)  ;
\end{scope}
\end{tikzpicture}


==> SeriesModelDiagram.tex <==
\begin{tikzpicture}	[auto]
\tikzstyle{LineOut}   = [ draw=black,  thick, o-]
\tikzstyle{LineIn}   = [ draw=black,  thick, -o]
\tikzstyle{LittleArrow}= [draw=black, thin, ->]
\tikzstyle{Block}=[rectangle, draw=black, thick, text width=5em, text centered, sharp corners]
	\node [matrix, column sep=12mm, row sep=7mm] (SeriesModels){ 
		\node  (Noden) {$v_n$}; & \node [Block] (Anm) {$A_{nm}$}; & \node (Nodem){$v_m$}; \\
};
\begin{scope}
\path [LineOut](Noden.east) -- node [name=MidwayNode, midway, yshift=2mm] {$i_{nm}$}  (Anm.west); 
\path [LineIn] (Anm.east) -- (Nodem.west);
\draw ($(MidwayNode.south)$) node [yshift=-0.5mm] {$\rightarrow$}  ; 
\end{scope}
\end{tikzpicture}


==> TrLineDiagram.tex <==
\begin{tikzpicture}
\tikzstyle{LineOut}   = [ draw=black,  thick, o-]
\tikzstyle{LineIn}   = [ draw=black,  thick, -o]
\tikzstyle{LittleArrow}= [draw=black, thin, ->]
\tikzstyle{Block}=[rectangle, draw=black, thick, text width=5em, text centered, sharp corners]
	\node [matrix, ampersand replacement=\&, column sep=12mm, row sep=1mm] (SeriesModels){ 
		\node  (Noden) {$v_n$}; \& \node [Block] (Znm) {$Z_{nm}$}; \& \node (Nodem){$v_m$}; \\
};
\begin{scope}
\path [LineOut](Noden.east) -- node [name=MidwayNode, midway, yshift=4mm] {$i_{nm}$}  (Znm.west); 
\path [LineIn] (Znm.east) -- (Nodem.west);
\draw ($(MidwayNode.south)$) node [yshift=-0.5mm] {$\rightarrow$}; 
\end{scope}
\end{tikzpicture}

